A Formal Modular Synthesis Approach for the Coordination of 3-D Robotic Construction with Multi-robots

In this paper, we deal with the problem of coordinating multiple robots to build 3-D structures. This problem consists of a set of mobile robots that interact with each other in order to autonomously build a predefined 3-D structure. Our approach is based on Supervisory Control Theory, and it allows us to synthesize from models that represent a single robot and the target structure a correct-by-construction reactive controller, called supervisor. When this supervisor is replicated for the other robots, then the target structure can be completed by all robots

==> bkp/step.tex <==
\begin{figure*}[ht!]
	\centering
	\def\myScale{.74}
	\def\mytrim{2cm 0 2cm 0}
	\subfigure[{$\St[0]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/S0.eps}
		\label{img:S0}
	}
	\subfigure[{$\St[0]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/S0a.eps}
		\label{img:S0a}
	}
	\subfigure[{$\St[1]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/S1.eps}
		\label{img:S1}
	}
	\subfigure[{$\St[2]$}]{
		\includegraphics[scale = \myScale, trim =  1.5cm 0 1.5cm 0 ]{img/exSteps/S2.eps}
		\label{img:S2}
	}
	\subfigure[{$\St[2]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/S2a.eps}
		\label{img:S2a}
	}
	\subfigure[{$\St[3]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/S3.eps}
		\label{img:S3}
	}
	\subfigure[{$\St[3]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/S3a.eps}
		\label{img:S3a}
	}
	\subfigure[{$\St[4]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/S4.eps}
		\label{img:S4}
	}
	\subfigure[{$\St[k]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/Sn.eps}
		\label{img:Sk}
	}
	\subfigure[{$\St[k+1]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/Sbad.eps}
		\label{img:Sbad}
	}
	\subfigure[{$\St[k]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/Sna.eps}
		\label{img:Sna}
	}
	\subfigure[{$\St[k+1]$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/Sgood.eps}
		\label{img:Sgood}
	}
	\subfigure[{$\St$}]{
		\includegraphics[scale = \myScale, trim = 1.5cm 0 1.5cm 0]{img/exSteps/Sn_1.eps}
		\label{img:S}
	}
	%
	\caption{Construction of the target $\St$  with three construction robots}
	\label{img:exSBS}
\end{figure*}


==> img/remove.tex <==
\psfrag{S0}{}

==> img/rename.tex <==
%\def\ftsmall{\fontsize{4}{12} \selectfont}
\def\sizeEvent{\scriptsize}
\def\sizeState{\scriptsize}
\def\sizeGuard{\scriptsize}

% grid
\psfrag{loc}{\tiny $\loc[i \bcom j]$}


%events

\psfrag{gb}{\sizeEvent $p$}
\psfrag{in}{\sizeEvent $in :$ }
\psfrag{out}{\sizeEvent $out:$}
\psfrag{r}{\sizeEvent $e:$}
\psfrag{l}{\sizeEvent $w:$}
\psfrag{u}{\sizeEvent $n:$}
\psfrag{d}{\sizeEvent $s:$}
\psfrag{aij}{\sizeEvent $a_{ij}:$}
\psfrag{aijset}{\sizeEvent $a_{11}\bcom \cdots \bcom a_{NM}$}
\psfrag{aisjs}{\sizeEvent $a_{i_sj_s}:$}
\psfrag{a_ij}{\sizeEvent $\{a_{ij} \bcom \cdots \bcom a_{NM}\} \setminus \{a_{i_sj_s}\}$}
\psfrag{aij1}{\sizeEvent $a_{i(j+1)}:$}
\psfrag{ai1j}{\sizeEvent $a_{(i+1)j}:$}

%guards

\psfrag{x >1}{\sizeGuard $y > 1$}
\psfrag{x < 2}{\sizeGuard $y < N$}
\psfrag{y>1}{\sizeGuard $x > 1$}
\psfrag{y< 3}{\sizeGuard $x < M$}
\psfrag{gout}{\sizeGuard $g_1$}
\psfrag{gviz}{\sizeGuard $g_2$}
\psfrag{hisjs == Hisjs -1}{\sizeGuard $h_{i_sj_s} = 0$}
\psfrag{hij == Hij - 1}{\sizeGuard $h_{ij} = h_{S_f}{ (i \bcom j)} - 1$}
\psfrag{hij < Hij - 1}{\sizeGuard $h_{ij} < h_{S_f}{(i \bcom j)} - 1$}

\psfrag{pos_ij = 0}{\sizeGuard $(x \ne i \lor y \ne j) \lor$}
\psfrag{modij1 = 0}{\sizeGuard $ |h_{ij} - h_{i(j+1)}| \le 1$}
\psfrag{pos_ij1 = 0}{\sizeGuard $(x \ne i \lor y \ne j + 1) \lor$}
\psfrag{posi1j = 0}{\sizeGuard $(x \ne i + 1 \lor y \ne j ) \lor$}

\psfrag{modi1j = 0}{\sizeGuard $ |h_{ij} - h_{(i+1)j}| \le 1$}

\psfrag{hij >= hij-1}{\sizeGuard $ h_{ij} \ge h_{i'j'}  \lor  h_{ij} \ge h_{i''j''}$}
%\psfrag{hij >= hij-1  |  hij >= hij+1}{\sizeGuard $ h_{ij} \ge h_{i(j-1)}  \lor  h_{ij} \ge h_{i(j+1)}$}

\psfrag{hij_ij1}{\sizeGuard $\lnot (x = i \land (y = j \lor y = j+1)) \lor (h_{ij} = h_{i(j+1)})$}
\psfrag{hij_i1j}{\sizeGuard $\lnot ((x = i \lor x = i+1) \land y = j) \lor (h_{ij} = h_{(i+1)j})$}

% Emove
\psfrag{gr = 0}{\sizeGuard $ g_e$}
\psfrag{gl = 0}{\sizeGuard $ g_w $}
\psfrag{gu = 0}{\sizeGuard $ g_n $}
\psfrag{gd = 0}{\sizeGuard $ g_s $}
\psfrag{go = 0}{\sizeGuard $ g_{out} $}
\psfrag{gi = 0}{\sizeGuard $ g_{in} $}
%Ehij
\psfrag{ga11}{\sizeGuard $(i \bcom j) \in \N[xy] \land h_{xy} = h_{ij}$}

%update
\psfrag{x = 1}{\sizeGuard $x:= i_s $}
\psfrag{y = 1}{\sizeGuard $y := j_s$}
\psfrag{x += 1}{\sizeGuard $y := y + 1$}
\psfrag{y +=1}{\sizeGuard $x := x + 1$}
\psfrag{x -= 1}{\sizeGuard $y := y - 1$}
\psfrag{y-=1}{\sizeGuard $x:= x - 1$}

\psfrag{x = 0}{\sizeGuard $x := 0 $}
\psfrag{y = 0}{\sizeGuard $y := 0$}
\psfrag{hij += 1}{\sizeGuard $h_{ij} := h_{ij} + 1$}

%states

\psfrag{q0}{\sizeState $\state[0]$}
\psfrag{q1}{\sizeState $\state[1]$}
\psfrag{L1}{}
\psfrag{S0}{}
\psfrag{S1}{}
\psfrag{B0}{}
\psfrag{B1}{}


\psfrag{G1}{\footnotesize $\Gv[1]:$}
\psfrag{G2}{\footnotesize $\Gv[2]:$}
\psfrag{G3}{\footnotesize $\Gv[3]:$}
\psfrag{G4}{\footnotesize $\Gv[4]:$}
\psfrag{Gin}{\footnotesize $\Gv[5]:$}
\psfrag{G5}{\footnotesize $\Gv[6]:$}
\psfrag{G6}{\footnotesize $\Gv[7]:$}
\psfrag{G8}{\footnotesize $\Gv[8]:$}
\psfrag{G9}{\footnotesize $\Gv[9]:$}
